Separating the Expressive Power of Propositional Dynamic and Modal Fixpoint Logics

We investigate the expressive power of the two main kinds of program logics for complex, non-regular program properties found in the literature: those extending propositional dynamic logic (PDL), and those extending the modal mu-calculus. This is inspired by the recent discovery of a decidable program logic called Visibly Pushdown Fixpoint Logic with Chop which extends both the modal mu-calculus and PDL over visibly pushdown languages, which, so far, constituted the ends of two pillars of decidable program logics. Here we show that this logic is not only more expressive than either of its two fragments, but in fact even more expressive than their union. Hence, the decidability border amongst program logics has been properly pushed up. We complete the picture by providing results separating all the PDL-based and modal fixpoint logics with regular, visibly pushdown and arbitrary context-free constructions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{10}
\providecommand{\publicationstatus}{V. Castiglioni and O. Dardha (Eds.): Combined Workshop on \\Expressiveness in Concurrency and Structural Operational Semantics \\ (EXPRESS/SOS 2021)\\
EPTCS 339, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.339.4}{10.4204/EPTCS.339.4}}

